Odd Khovanov homology for tangles

We extend the covering of even and odd Khovanov link homology to tangles, using arc algebras. For this, we develop the theory of quasi-associative algebras and bimodules graded over a category with a 3-cocycle. Furthermore, we show that a covering version of a level 2 cyclotomic half 2-Kac--Moody algebra acts on the bicategory of quasi-associative bimodules over the covering arc algebras, relating our work to a construction of Vaz.

==> pictures/cobcornersW.tex <==
\tikzdiagc[scale=.75]{
	\filldraw [fill=white, draw=black] (.5,1.25) rectangle (4,3.75);
	\draw (-1,2.75) -- (.5,3.75);
	%
	%
	\draw (0,0) .. controls (0,.-.25) and (1,-.25) .. (1,0);
	\draw[dashed] (0,0) .. controls (0,.25) and (1,.25) .. (1,0);
	%
	\draw (0,0) -- (0,4);
	\draw (1,0) -- (1,4);
	%
	\draw (0,4) .. controls (0,3.75) and (1,3.75) .. (1,4);
	\draw (0,4) .. controls (0,4.25) and (1,4.25) .. (1,4);
	%
	\node at(1.5,.25) {\tiny $\dots$};
	\node at(1.5,3.75) {\tiny $\dots$};
	%
	\draw (2,0) .. controls (2,.-.25) and (3,-.25) .. (3,0);
	\draw[dashed] (2,0) .. controls (2,.25) and (3,.25) .. (3,0);
	%
	\draw (2,0) -- (2,4);
	\draw (3,0) -- (3,4);
	%
	\draw (2,4) .. controls (2,3.75) and (3,3.75) .. (3,4);
	\draw (2,4) .. controls (2,4.25) and (3,4.25) .. (3,4);
	%
	%
	%\draw (-1,2.25) rectangle (5,3.25);
	%\draw (-2,.75) rectangle (4,1.75);
	%
	%
	\filldraw [fill=white, draw=black] (3,2.75) -- (4,3.75) -- (4,1.25) -- (3,.25);
	\filldraw [fill=white, draw=black] (-1,.25) rectangle (3,2.75);
	%\filldraw [fill=white, draw=black,rounded corners] (-.5,.5) rectangle (3.5,3.5) node[midway] { $W$};
}

==> pictures/ndeath.tex <==
\tikzdiag[xscale=-.75,yscale=.75]{0}{
	\draw (1,0) .. controls (1,1) and (2,1) .. (2,0);
	%
	\draw (1,0) .. controls (1,-.25) and (2,-.25) .. (2,0);
	\draw[dashed] (1,0) .. controls (1,.25) and (2,.25) .. (2,0);
	%
	\draw[->] (1.5,1.5) [partial ellipse=0:270:2ex and 1ex];
}
